Types of Fireballs (Extended Version)

The good properties of Plotkin's call-by-value lambda-calculus crucially rely on the restriction to weak evaluation and closed terms. Open call-by-value is the more general setting where evaluation is weak but terms may be open. Such an extension is delicate, and the literature contains a number of proposals. Recently, Accattoli and Guerrieri provided detailed operational and implementative studies of these proposals, showing that they are equivalent from the point of view of termination, and also at the level of time cost models. This paper explores the denotational semantics of open call-by-value, adapting de Carvalho's analysis of call-by-name via multi types (aka non-idempotent intersection types). Our type system characterises normalisation and thus provides an adequate relational semantics. Moreover, type derivations carry quantitative information about the cost of evaluation: their size bounds the number of evaluation steps and the size of the normal form, and we also characterise derivations giving exact bounds. The study crucially relies on a new, refined presentation of the fireball calculus, the simplest proposal for open call-by-value, that is more apt to denotational investigations.

==> normal-forms-typable-tight.tex <==
% !TEX root = ../main.tex
\begin{proof}
Two cases, either $\expr$ is a fireball or a normal program.
\begin{itemize}
\item \emph{$\expr$ is a fireball $\fire$}. By induction on the definition of fireballs. 
Note that if $\fire$ is a value the statement is given by \reflemmap{value-typing}{judg}. 
Therefore, suppose that $\fire$ is a inert term of the form $\var \fire_1 \ldots \fire_n$. 
By \ih, $\fire_i$ is typable with a tight derivation $\concl{\tdertwo_i}{\typctxtwo_i}{\fire_i}{\emptymset}$. 
The tight derivation $\tder$ is then constructed as follows. Let $\ptype_1 \defeq \ptype$ and $\ptype_{k+1} \defeq \mset{\Pair\emptymset {\ptype_k}}$. 
Note that $\ptype_k$ is a tight type. We use $\ptype_{n+1}$ for the type of $\var$:
  \begin{equation*}
    \tder \defeq 
    \AxiomC{}
    \RightLabel{\footnotesize$\ruleAx$}
    \UnaryInfC{$\var \hastype \ptype_{n+1}  \vdash \var \hastype \ptype_{n+1}$}
    \AxiomC{$\ \vdots\,\tdertwo_1$}
    \noLine
    \UnaryInfC{$\typctxtwo_1 \vdash \fire_1 \hastype \emptymset$}
    \RightLabel{\footnotesize$\ruleAp$}
    \BinaryInfC{$\var \hastype  \ptype_{n+1}  \uplus \typctxtwo_1  \vdash \var \fire_1 \hastype  \ptype_n$}
    \UnaryInfC{$\vdots$}
        \AxiomC{$\ \vdots\,\tdertwo_n$}
    \noLine
    \UnaryInfC{$\typctxtwo_n \vdash \fire_n \hastype \emptymset$}
    \RightLabel{\footnotesize$@$}
    \BinaryInfC{$\var \hastype \mset{ \ptype_{n+1}}  \uplus (\biguplus_{i=1}^n\typctxtwo_i ) \vdash \var \fire_1 \ldots \fire_n \hastype \ptype_1$}
    \DisplayProof
  \end{equation*}

	\item \emph{$\expr$ is a normal program $\prog$}. 
	By induction on the length $n$ of the environment in $\prog$. 
	If $n=0$ then $\prog = (\fire, \emptyenv)$ and we apply the case for fireballs (adding the rule $\EsCoerc$ at the end of the type derivation). 
	Otherwise $n>0$ and $\prog = (\fire, \genv\appendOp\esub\var\itm)$. 
	By \ih, there is a tight derivation $\concl{\tderthree}{\typctxthree, \var\hastype \ptype}{(\fire, \genv)}{\emptymset}$, for some positive type $\ptype$. 
% 	We assume that $\var \in \Dom\typctxthree$, because if it does not then then we can extend the typing context with $\var \hastype \emptymset$ using weakening (\reflemmap{weakening}{add}) and without changing the size of the derivation (nor its tightness). Therefore, let 
%     Let $\typctxthree = \typctxthree', \var\hastype \ptype$. 
    By \ih, there is a tight derivation $\concl{\tdertwo}{\typctxtwo}{\itm}{\ptype}$. The tight derivation $\tder$ is then constructed as follows:
    \begin{equation*}
        \tder \defeq
        \AxiomC{$\ \vdots\, \tderthree$}
        \noLine
        \UnaryInfC{$\typctxthree, \var \hastype \ptype \vdash (\fire, \genv) \hastype \emptymset$}
        \AxiomC{$\ \vdots\, \tdertwo$}
        \noLine
        \UnaryInfC{$\typctxtwo\vdash \itm \hastype \ptype$}
         \RightLabel{\footnotesize$\EsAppend$}
         \BinaryInfC{$\typctxthree \uplus \typctxtwo \vdash (\fire, \genv \appendOp \esub\var\itm) \hastype \emptymset$}
        \DisplayProof
    \end{equation*}
    \qedhere
\end{itemize}
\end{proof}


==> proofs-normal-forms-tight.tex <==
\subsection{Omitted proofs and lemmas of \refsect{tight}}

\setcounter{lemmaAppendix}{\value{l:tight-ctx-imply-tight-type}}
\begin{lemmaAppendix}[Being tight is spine-hereditary]
\label{lappendix:tight-ctx-imply-tight-type}
\NoteState{l:tight-ctx-imply-tight-type}
Let $\concl{\tder}{\typctx}{\itm}{\ptype}$ be a derivation and $\typctx$ be a tight typing context. Then $\ptype$ (and so $\tder$) is tight.
\end{lemmaAppendix}

\begin{proof}
By induction on the structure of $\itm$. If $\itm = \var$ then $\typctx$ contains the assignment $\var \hastype \ptype$. Then $\ptype$ is tight because $\typctx$ is tight. If $\itm = \itmtwo \fire$ then $\tder$ has the form:
		    \begin{equation*}
	\AxiomC{$\ \vdots\, \tdertwo$}
        \noLine
        \UnaryInfC{$\typctxthree \vdash \itmtwo \hastype \mset{\Pair{\ptypetwo}{\ptype}}$}
        \AxiomC{$\ \vdots\, \tderthree$}
        \noLine
        \UnaryInfC{$\typctxtwo\vdash \fire \hastype \ptypetwo$}
         \RightLabel{\footnotesize$\EsAppend$}
         \BinaryInfC{$\typctxthree \uplus \typctxtwo \vdash \itmtwo\fire \hastype \ptype$}
        \DisplayProof
      \end{equation*}
with $\typctx = \typctxthree \uplus \typctxtwo$. Then $\typctxthree$ is tight because $\typctx$ is tight. By applying the \ih to $\tdertwo$ we obtain that $\mset{\Pair{\ptypetwo}{\ptype}}$ is tight, that implies that $\ptype$ is tight.
\end{proof}

\setcounter{lemmaAppendix}{\value{l:size-normal-tight}}
\begin{lemmaAppendix}[Tight derivations are minimal and provide the exact size of normal forms]
\label{lappendix:size-normal-tight} % \reflemmap{size-normal}{tight}
\NoteState{l:size-normal-tight}
Let $\concl{\tder}{\typctx}{\expr}{\ptype}$ be a tight derivation and $\expr$ be a normal %program or a fireball
expression. 
%If $\tder$ is tight then 
Then $\sizeap\expr = \sizeap\tder$ and $\size{\tder}$ is minimal among the typing derivations of $\expr$.
\end{lemmaAppendix}

\begin{proof}
Minimality of $\size{\tder}$ follows from the fact that $\sizeap{\expr} = \sizeap{\tder}$ and \refprop{size-normal}.
We prove that $\sizeap{\expr} = \sizeap{\tder}$ by induction on $\expr$. 
\begin{itemize}
    \item \emph{$\expr$ is a value}. 
    We have $\ptype = \emptymset$, since $\tder$ is tight. Then the statement follows by \reflemmap{value-typing}{empty}.

    \item \emph{$\expr$ is a inert term}. Then $\expr = \var \fire_1 \ldots \fire_n$ (for some $n > 0$) and $\tder$ has the form:
    {\small
  \begin{equation*}
    \AxiomC{}
    \RightLabel{\footnotesize$\ruleAx$}
    \UnaryInfC{$\var \hastype \mset{\Pair{\ptypetwo_1}{\mset{\Pair{\ldots}{\mset{\Pair{\ptypetwo_n}{\ptype}}}}}}  \vdash \var \hastype \mset{\Pair{\ptypetwo_1}{\mset{\Pair{\ldots}{\mset{\Pair{\ptypetwo_n}{\ptype}}}}}}$}
    \AxiomC{$\ \vdots\,\tdertwo_1$}
    \noLine
    \UnaryInfC{$\typctxtwo_1 \vdash \fire_1 \hastype \ptypetwo_1$}
    \RightLabel{\footnotesize$\ruleAp$}
    \BinaryInfC{$\var \hastype  \mset{\Pair{\ptypetwo_1}{\mset{\Pair{\ldots}{\mset{\Pair{\ptypetwo_n}{\ptype}}}}}}  \uplus \typctxtwo_1  \vdash \var \fire_1 \hastype  \mset{\Pair{\ptypetwo_2}{\mset{\Pair{\ldots}{\mset{\Pair{\ptypetwo_n}{\ptype}}}}}}$}
    \UnaryInfC{$\vdots$}
        \AxiomC{$\ \vdots\,\tdertwo_n$}
    \noLine
    \UnaryInfC{$\typctxtwo_n \vdash \fire_n \hastype \ptypetwo_n$}
    \RightLabel{\footnotesize$@$}
    \BinaryInfC{$\var \hastype \mset{\Pair{\ptypetwo_1}{\mset{\Pair{\ldots}{\mset{\Pair{\ptypetwo_n}{\ptype}}}}}}  \uplus (\biguplus_{i=1}^n\typctxtwo_i ) \vdash \var \fire_1 \ldots \fire_n \hastype \ptype$}
    \DisplayProof
  \end{equation*}
  }
  
    Since $\tder$ is tight, $\ptypetwo_1 = \ldots = \ptypetwo_n = \emptymset$ and all the types in $\typctxtwo_1, \ldots, \typctxtwo_n$ are tight. 
    Therefore, all the derivations $\concl{\tdertwo_i}{\typctxtwo_i}{\fire_i}{\emptymset}$ are tight. 
    Then $\sizeap{\fire_i} = \sizeap{\tdertwo_i}$ by \ih, and so $\sizeap{\expr} = \sizeap{\var \fire_1 \ldots \fire_n} = n + \sum_{i=1}^n\sizeap{\fire_i} = n + \sum_{i=1}^n\sizeap{\tder_i} = \sizeap\tder$..

	\item \emph{$\expr$ is a program $\prog$}. By induction on the length $n$ of the environment. If $n=0$ then $\prog = (\fire, \emptyenv)$ and we apply the case for fireballs. Otherwise $n>0$ and $\prog = (\fire, \genv\appendOp\esub\var\itm)$. Then $\tder$ has the following form:
		    \begin{equation*}
	\AxiomC{$\ \vdots\, \tdertwo$}
        \noLine
        \UnaryInfC{$\typctxthree, \var \hastype \ptypetwo \vdash (\fire, \genv) \hastype \ptype$}
        \AxiomC{$\ \vdots\, \tderthree$}
        \noLine
        \UnaryInfC{$\typctxtwo\vdash \itm \hastype \ptypetwo$}
         \RightLabel{\footnotesize$\EsAppend$}
         \BinaryInfC{$\typctxthree \uplus \typctxtwo \vdash (\fire, \genv \appendOp \esub\var\itm) \hastype \ptype$}
        \DisplayProof
      \end{equation*}
with $\typctx = \typctxthree \uplus \typctxtwo$. 
    Note that $\typctxtwo$ and $\typctxthree$ are tight because $\typctx$ is tight. By \reflemma{tight-ctx-imply-tight-type}, $\ptypetwo$ is tight, and so both $\tdertwo$ and $\tderthree$ are tight. Then $\sizeap{(\fire, \genv)} = \sizeap\tdertwo$ and $\sizeap \itm = \sizeap\tderthree$ by \ih, and so $\sizeap \expr = \sizeap{(\fire, \genv \appendOp \esub\var\itm)} = \sizeap{(\fire, \genv)} + \sizeap \itm = \sizeap\tdertwo + \sizeap\tderthree = \sizeap\tder$.
    \qedhere
	\end{itemize}
\end{proof}

\setcounter{propositionAppendix}{\value{prop:characterization-nfs}}
\begin{propositionAppendix}[Tight type characterization of normal forms]
\label{propappendix:characterization-nfs}
\NoteState{prop:characterization-nfs}
  Let $\expr$ be a normal expression. 
  Then, there exist a tight type contexts $\typctx$ and a tight type derivation $\concl{\tder}{\typctx}{\expr}{\emptymset}$.
%   More precisely, there are only two possibilities for $\expr$:
%   \begin{itemize}
%     \item $\expr$ is a \valu\ or coerced \valu, and there is a (tight) type derivation $\concl{\tder}{\ }{\expr}{\emptymset}$;
%     \item $\expr$ contains an inert term, and for any tight type $\ptype$ there are a tight type context $\typctx$ and a (tight) type derivation $\concl{\tder}{\typctx}{\expr}{\ptype}$ with $\domain{\typctx} \neq \emptyset$.
%   \end{itemize}
  More precisely, there are only three possibilities for~$\expr$:
  \begin{enumerate}
    \item $\expr$ is a \valu\ or coerced \valu, and there is a (tight) type derivation $\concl{\tder}{\ }{\expr}{\emptymset}$;
    \item $\expr$ is a pseudo-\valu, and there is a (tight) type derivation $\concl{\tder}{\typctx}{\expr}{\emptymset}$ where $\typctx$ is a tight type context such that $\domain{\typctx} \neq \emptyset$;
    \item $\expr$ %contains an inert term
    is hereditarily inert, and for any tight multi type $\ptype$ there are a tight type context $\typctx$ and a (tight) type derivation $\concl{\tder}{\typctx}{\expr}{\ptype}$ with $\domain{\typctx} \neq \emptyset$.
    \end{enumerate}
\end{propositionAppendix}

\begin{proof}
Two cases, either $\expr$ is a fireball or a normal program.
\begin{itemize}
\item \emph{$\expr$ is a fireball $\fire$}. By induction on the definition of fireballs. 
Note that if $\fire$ is a \valu\ the statement is given by \reflemmap{value-typing}{judg}. 
Therefore, suppose that $\fire$ is an term of the form $\var \fire_1 \ldots \fire_n$ ($n > 0$). 
By \ih, $\fire_i$ is typable with a tight type derivation $\concl{\tdertwo_i}{\typctxtwo_i}{\fire_i}{\emptymset}$ (for all $0 \leq i \leq n$). 
The tight type derivation $\tder$ is then constructed as follows. 
Let $\ptype_1 \defeq \ptype$ and $\ptype_{i+1} \defeq \mset{\Pair\emptymset {\ptype_i}}$ (for all $1 \leq i \leq n$). 
Note that all $\ptype_i$'s and $\typctxtwo_i$'s are tight and hence $\var \hastype \ptype_{n+1} \uplus (\biguplus_{i=1}^n\typctxtwo_i )$ is tight, moreover $\domain{\var \hastype \ptype_{n+1} \uplus (\biguplus_{i=1}^n\typctxtwo_i )} \neq \emptyset$ because of $\ptype_{n+1}$. 
% We use $\ptype_{n+1}$ for the type of $\var$:
  \begin{equation*}
    \tder \defeq 
    \AxiomC{}
    \RightLabel{\footnotesize$\ruleAx$}
    \UnaryInfC{$\var \hastype \ptype_{n+1}  \vdash \var \hastype \ptype_{n+1}$}
    \AxiomC{$\ \vdots\,\tdertwo_1$}
    \noLine
    \UnaryInfC{$\typctxtwo_1 \vdash \fire_1 \hastype \emptymset$}
    \RightLabel{\footnotesize$\ruleAp$}
    \BinaryInfC{$\var \hastype  \ptype_{n+1}  \uplus \typctxtwo_1  \vdash \var \fire_1 \hastype  \ptype_n$}
    \UnaryInfC{$\vdots$}
        \AxiomC{$\ \vdots\,\tdertwo_n$}
    \noLine
    \UnaryInfC{$\typctxtwo_n \vdash \fire_n \hastype \emptymset$}
    \RightLabel{\footnotesize$@$}
    \BinaryInfC{$\var \hastype \ptype_{n+1} \uplus (\biguplus_{i=1}^n\typctxtwo_i ) \vdash \var \fire_1 \ldots \fire_n \hastype \ptype_1$}
    \DisplayProof
  \end{equation*}

	\item \emph{$\expr$ is a normal program $\prog$}. 
	By induction on the length $n$ of the environment in $\prog$. 
	If $n=0$ then $\prog = (\fire, \emptyenv)$ and we apply the case for fireballs (adding the rule $\EsCoerc$ at the end of the type derivation, which preserves all types). 
	Otherwise $n>0$ and $\prog = (\fire, \genv\appendOp\esub\var\itm)$. 
	By \ih, there is a tight derivation $\concl{\tderthree}{\typctxthree, \var\hastype \ptypetwo}{(\fire, \genv)}{\ptype}$ (where $\ptype = \emptymset$ if $\fire$ is a \valu), for some tight multi type $\ptypetwo$ and some tight type context $\typctxthree$ (and $\domain{\typctxthree, \var \hastype \ptypetwo} \neq \emptyset$ if $(\fire, \genv)$ is a pseudo-\valu\ or hereditarily inert). 
% 	We assume that $\var \in \Dom\typctxthree$, because if it does not then then we can extend the typing context with $\var \hastype \emptymset$ using weakening (\reflemmap{weakening}{add}) and without changing the size of the derivation (nor its tightness). Therefore, let 
%     Let $\typctxthree = \typctxthree', \var\hastype \ptype$. 
    By \ih, there is a tight derivation $\concl{\tdertwo}{\typctxtwo}{\itm}{\ptypetwo}$ for some tight type context $\typctxtwo$ with $\domain{\typctxtwo} \neq \emptyset$. 
    The tight derivation $\tder$ is then 
    constructed as follows (note that $\domain{\typctxthree \uplus \typctxtwo} \neq \emptyset$):
    \begin{equation*}
        \tder \defeq
        \AxiomC{$\ \vdots\, \tderthree$}
        \noLine
        \UnaryInfC{$\typctxthree, \var \hastype \ptypetwo \vdash (\fire, \genv) \hastype \ptype$}
        \AxiomC{$\ \vdots\, \tdertwo$}
        \noLine
        \UnaryInfC{$\typctxtwo\vdash \itm \hastype \ptypetwo$}
         \RightLabel{\footnotesize$\EsAppend$}
         \BinaryInfC{$\typctxthree \uplus \typctxtwo \vdash (\fire, \genv \appendOp \esub\var\itm) \hastype \ptype$}
        \DisplayProof
    \end{equation*}
    \qedhere
\end{itemize}
\end{proof}

\setcounter{propositionAppendix}{\value{prop:tight-types-bound-nfs}}
\begin{propositionAppendix}[Tight types give the exact size of normal forms]
\label{propappendix:tight-types-bound-nfs}
\NoteState{prop:tight-types-bound-nfs}
  Let $\expr$ be a normal expression and $\concl{\tder}{\typctx}{\expr}{\emptymset}$ be a tight derivation. Then $\sizeap{\expr} = \size{\typelist\typctx}$.
\end{propositionAppendix}

\begin{proof}
In order to have the right \ih, we prove a stronger statement:
  Let $\expr$ be a normal expression and $\concl{\tder}{\typctx}{\expr}{\ptype}$ be a tight type derivation.
  \begin{itemize}
    \item If $\ptype = \emptymset$ then $\sizeap{\expr} = \size{\typelist\typctx}$.
    \item If $\expr$ is an inert term, then $\sizeap{\expr} + \size{\ptype} = \size{\typelist\typctx}$.
  \end{itemize}

In the proof of this stronger statement there are two cases: either $\expr$ is a fireball or a normal program.
% Note that $\sizeap{\expr} + \size{\ptype}\leq \size{\typelist\typctx}$ implies $\sizeap{\expr} \leq \size{(\typelist\typctx, \ptype)}$.

\begin{itemize}
\item \emph{$\expr$ is a fireball $\fire$}. By induction on the definition of fireballs. 
If $\fire$ is a value then $\domain{\typctx} = \emptyset$ according to the tight type characterization of normal forms (\refprop{characterization-nfs}), hence $\sizeap{\expr} = 0 = \size{\typelist\typctx}$. 
Otherwise $\fire$ is a inert term of the form $\var \fire_1 \ldots \fire_n$ ($n > 0$). 
Any tight type derivation $\concl{\tder}{\typctx}{\var \fire_1 \ldots \fire_n}{\ptype}$ is constructed as follows, where $\ptypetwo_1 \defeq \ptype$, $\ptypetwo_{i+1} \defeq \mset{\Pair{\emptymset}{\ptypetwo_i}}$ ($1 \leq i \leq n$) and $\typctx = \var \hastype \ptypetwo_{n+1}  \uplus (\biguplus_{i=1}^n\typctxtwo_i)$ (note that the tightness of $\typctx$ has many implications!):
  \begin{equation*}
    \tder \defeq 
    \AxiomC{}
    \RightLabel{\footnotesize$\ruleAx$}
    \UnaryInfC{$\var \hastype \ptypetwo_{n+1}  \vdash \var \hastype \ptypetwo_{n+1}$}
    \AxiomC{$\ \vdots\,\tdertwo_1$}
    \noLine
    \UnaryInfC{$\typctxtwo_1 \vdash \fire_1 \hastype \emptymset$}
    \RightLabel{\footnotesize$\ruleAp$}
    \BinaryInfC{$\var \hastype  \ptypetwo_{n+1}  \uplus \typctxtwo_1  \vdash \var \fire_1 \hastype  \ptypetwo_n$}
    \UnaryInfC{$\vdots$}
        \AxiomC{$\ \vdots\,\tdertwo_n$}
    \noLine
    \UnaryInfC{$\typctxtwo_n \vdash \fire_n \hastype \emptymset$}
    \RightLabel{\footnotesize$@$}
    \BinaryInfC{$\var \hastype \ptypetwo_{n+1}  \uplus (\biguplus_{i=1}^n\typctxtwo_i ) \vdash \var \fire_1 \ldots \fire_n \hastype \ptypetwo_1$}
    \DisplayProof
  \end{equation*}
    By \ih, $\sizeap{\fire_i} = \size{\typelist\typctxtwo_i}$.
    Note that $\size{\ptypetwo_{n+1}} = n + \size{\ptype}$. 
    Therefore, $\sizeap{\var \fire_1\dots\fire_n} + \size{\ptypetwo_1} = n + \sum_i^n\sizeap{\fire_i} + \size{\ptypetwo_1} = n + \sum_i^n \size{\typelist\typctxtwo_i} + \size{\ptypetwo_1} =\size{\typelist{\var \hastype \ptypetwo_{n+1}  \uplus (\biguplus_{i=1}^n\typctxtwo_i )}}$.

	\item \emph{$\expr$ is a program $\prog$}. 
	By induction on the length $n$ of the environment in $\prog$. 
	If $n=0$ then $\prog = (\fire, \emptyenv)$ and the last rule of any type derivation for $\prog$ is $\EsCoerc$ (which preserves types), thus we can apply the case for fireballs, since $\sizeap{(\fire, \emptyenv)} = \sizeap{\fire}$. 
	Otherwise $n>0$ and $\prog = (\fire, \genv\appendOp\esub\var\itm)$. 
	Any tight type derivation $\concl{\tder}{\typctx}{\prog}{\emptymset}$ is then constructed as follows, where $\typctx = \typctxthree \uplus \typctxtwo$:
	    \begin{equation*}
        \tder \defeq
	\AxiomC{$\ \vdots\, \tderthree$}
        \noLine
        \UnaryInfC{$\typctxthree, \var \hastype \ptypetwo \vdash (\fire, \genv) \hastype \emptymset$}
        \AxiomC{$\ \vdots\, \tdertwo$}
        \noLine
        \UnaryInfC{$\typctxtwo\vdash \itm \hastype \ptypetwo$}
         \RightLabel{\footnotesize$\EsAppend$}
         \BinaryInfC{$\typctxthree \uplus \typctxtwo \vdash (\fire, \genv \appendOp \esub\var\itm) \hastype \emptymset$}
        \DisplayProof
      \end{equation*}
      Since $\typctxtwo$ is tight, then $\ptypetwo$ is tight by \reflemma{tight-ctx-imply-tight-type} applied to $\tdertwo$, hence $\tdertwo$ is tight.
      By \ih, $\sizeap{(\fire,\genv)} = 
      \size{\typelist{\typctxthree, \var \hastype \ptypetwo}}$ and $\sizeap{\itm} + \size{\ptypetwo} = \size{\typelist\typctxtwo}$. 
      Hence, $\sizeap{(\fire, \genv \appendOp \esub\var\itm)} = \sizeap{(\fire, \genv)} + \sizeap{\itm} = \size{\typelist{\typctxthree, \var \hastype \ptypetwo}} + \size{\typelist\typctxtwo} - \size{\ptypetwo} = \size{\typelist{\typctxthree \uplus \typctxtwo}}$.
      \qedhere
\end{itemize}
\end{proof}


\setcounter{theoremAppendix}{\value{thm:tight-correctness}}
\begin{theoremAppendix}[Tight correctness]
\label{thmappendix:tight-correctness}
\NoteState{thm:tight-correctness}
% Let $\concl{\tder}{\typctx}{\prog}{\emptymset}$ be a tight derivation. 
% Then there exists a normal form $\progtwo$ and a derivation $\deriv: \prog \tof^* \progtwo$ with $\size\deriv + \sizeap\progtwo = \sizeap\tder$.
Let $\concl{\tder}{\typctx}{\prog}{\emptymset}$ be a tight type derivation. Then there %are a normal form $\progtwo$ and a
is a normalizing evaluation $\deriv \colon \prog \tof^* \progtwo$ with 
% $\sizeap\tder = \size\deriv + \sizeap\progtwo$
%     \begin{equation}
%     \tag{\ref{eq:correctness}}
%     \sizeap\tder = \size\deriv + \sizeap\progtwo = \size\deriv + \sizeap{\typelist\typctx} \, .
%     \end{equation}
$    \sizeap\tder = \size\deriv + \sizeap\progtwo = \size\deriv + \sizeap{\typelist\typctx}$.
In particular, if $\domain{\typctx} = \emptyset$, then $\size{\tder} = \size{\deriv}$ and $\progtwo$ is a coerced value.
% For any type derivation $\concl{\tder}{\typctx}{\prog}{\emptymset}$ with $\typctx$ tight, there %are a normal form $\progtwo$ and a
% is a normalizing evaluation $\deriv: \prog \tof^* \progtwo$ with $\size\deriv + \sizeap\progtwo = \sizeap\tder$.
\end{theoremAppendix}

\begin{proof} 
% The second identity in \refeq{correctness} follows from the first one and \refprop{tight-types-bound-nfs}.
By induction on $\sizeap\tder$. 
If $\prog$ is normal then the statement holds with $\progtwo \defeq \prog$ and $\deriv$ the empty derivation ($\size{\deriv} = 0$), because $\tder$ and hence $\typctx$ are tight, so $\sizeap{\progtwo} = \sizeap{\tder}$ by \reflemma{size-normal-tight} and $\sizeap{\progtwo} = \sizeap{\typelist\typctx}$ by \refprop{tight-types-bound-nfs}. 
Otherwise $\prog \tof \progthree$ and by quantitative subject reduction (\refprop{quant-subject-reduction}) there is a tight derivation $\concl{\tdertwo}{\typctx}{\progthree}{\emptymset}$ such that $\sizeap\tdertwo = \sizeap\tder -1$. 
% Note that $\tder$ is tight since $\typctx$ is so.
By \ih, there exists $\progtwo$ normal and an evaluation $\derivtwo \colon \progthree \tof^* \progtwo$ such that $\size\derivtwo + \sizeap\progtwo = \sizeap\tdertwo$.
Then the evaluation $\deriv \colon \prog  \tof^* \progtwo$ obtained by prefixing $\derivtwo$ with the step $\prog \tof \progthree$ verifies $\size\deriv + \sizeap\progtwo = \size\derivtwo + 1 + \sizeap\progtwo = \sizeap\tdertwo + 1 = \sizeap\tder$.

If moreover $\domain{\typctx} = \emptyset$, then $\progtwo$ is a coerced value by \refprop{characterization-nfs}, so $\size{\progtwo} = 0$.
\end{proof}

\setcounter{theoremAppendix}{\value{thm:tight-completeness}}
\begin{theoremAppendix}[Tight completeness]
\label{thmappendix:tight-completeness}
\NoteState{thm:tight-completeness}
% Let $\deriv: \prog \tof^* \progtwo$ be a normalizing evaluation. 
% Then there is a tight type derivation $\concl{\tder}{\typctx}{\prog}{\emptymset}$ %, and it satisfies
% such that $\size\deriv + \sizeap\progtwo = \sizeap\tder$.
Let $\deriv \colon \prog \tof^* \progtwo$ be a normalizing evaluation. 
Then there is a tight type derivation $\concl{\tder}{\typctx}{\prog}{\emptymset}$ with 
% $\size\deriv + \sizeap\progtwo = \sizeap\tder$.
% \begin{equation}\tag{\ref{eq:completeness}}
%   \sizeap\tder = \size\deriv + \sizeap{\progtwo} = \size{\deriv} + \size{\typelist\typctx}\, .
% \end{equation}
$\sizeap\tder = \size\deriv + \sizeap{\progtwo} = \size{\deriv} + \size{\typelist\typctx}$.
In particular, if $\progtwo$ is a coerced value, then $\size{\tder} = \size{\deriv}$ and $\domain{\typctx} = \emptyset$. 
% Let $\deriv: \prog \tof^* \progtwo$ be a normalizing evaluation. 
% Then there is a type derivation $\concl{\tder}{\typctx}{\prog}{\emptymset}$ with $\typctx$ tight and $\size\deriv + \sizeap\progtwo = \sizeap\tder$.
\end{theoremAppendix}

\begin{proof}
  By induction on $\size\deriv$. If $\size\deriv = 0$ then $\prog = \progtwo$, so the existence of $\concl{\tder}{\typctx}{\prog}{\emptymset}$ with $\typctx$ tight is given by the fact that normal programs are tightly typable (\refprop{characterization-nfs}), and the equalities on sizes are given by \reflemma{size-normal-tight} and \refprop{tight-types-bound-nfs}. 
  If $\size\deriv  =k > 0$ then $\prog \tof \progthree \tof^k \progtwo$ and by \ih %we obtain a 
  there is a tight derivation $\concl{\tdertwo}{\typctx}{\progthree}{\emptymset}$ satisfying $k + \sizeap\progtwo = \sizeap\tdertwo$. 
  By quantitative subject expansion (\refprop{quant-subject-expansion}) there exists $\concl{\tder}{\typctx}{\prog}{\emptymset}$ %, satisfying
  with $\sizeap\tder = \sizeap\tdertwo +1$. Then $\size\deriv + \sizeap\progtwo = k + 1 + \sizeap\progtwo  =_{\ih} \sizeap\tdertwo + 1 = \sizeap\tder$.
  
  If moreover $\progtwo$ is a coerced value then $\size{\progtwo} = 0$ , and $\domain{\typctx} = \emptyset$ by \refprop{characterization-nfs}.
\end{proof}


